Prioritized Multi-View Stereo Depth Map Generation Using Confidence Prediction

In this work, we propose a novel approach to prioritize the depth map computation of multi-view stereo (MVS) to obtain compact 3D point clouds of high quality and completeness at low computational cost. Our prioritization approach operates before the MVS algorithm is executed and consists of two steps. In the first step, we aim to find a good set of matching partners for each view. In the second step, we rank the resulting view clusters (i.e. key views with matching partners) according to their impact on the fulfillment of desired quality parameters such as completeness, ground resolution and accuracy. Additional to geometric analysis, we use a novel machine learning technique for training a confidence predictor. The purpose of this confidence predictor is to estimate the chances of a successful depth reconstruction for each pixel in each image for one specific MVS algorithm based on the RGB images and the image constellation. The underlying machine learning technique does not require any ground truth or manually labeled data for training, but instead adapts ideas from depth map fusion for providing a supervision signal. The trained confidence predictor allows us to evaluate the quality of image constellations and their potential impact to the resulting 3D reconstruction and thus builds a solid foundation for our prioritization approach. In our experiments, we are thus able to reach more than 70% of the maximal reachable quality fulfillment using only 5% of the available images as key views. For evaluating our approach within and across different domains, we use two completely different scenarios, i.e. cultural heritage preservation and reconstruction of single family houses.

==> extending_mvs_confidence.tex <==
\subsection{Extending the MVS confidence to $k$ matching partners}
\label{sss:extended_mvs}
% In this subsection, we want to get from a unary MVS confidence
% Up to now the MVS confidence is learned and predicted for camera triplets (a key view and two matching partners).
% However, MVS typically works better with more than two matching partners.
In this subsection, we extend the confidence prediction to an arbitrary number of $k$ matching partners based 
on the individual unary MVS confidence predictions.
The basic assumption of this extension is that the MVS reconstruction process follows a stochastic process.
% Let us assume the MVS follows
%  a stochastic process.
Under this assumption, we can use probability theory to reason about 
 the overall probability of obtaining a successful measurement for a pixel of a key view 
 given a set of matching partners.
 For a successful measurement, most MVS approaches require successful matches to at least two matching partners.
 Thus, we can formulate the overall probability of obtaining a successful measurement, as the probability
 of getting successful matches to at least two matching partners.
In~\ref{conf_extension_appendix}, 
we derive this overall probability by growing a binary probability tree.
In the following, we apply the general solution described in~\ref{conf_extension_appendix} to our specific problem.

In our problem, we are given a surface mesh with a set of triangles $T$ and a set of images $C$.
For a specific combination of a key view $c_{key}\in C$ with $k$ matching partners $c^k \in C^k$,
we want to predict the chances of successfully reconstructing the depth of the pixels in which a triangle $t \in T$ projects.

% Thus let us set $d = k$ and rename
%  $P_{min 2} \mapsto f_{conf}(t,c_{key}, c^k)$ and  $p\left(c^{(i)}_a \right) \mapsto  f_{conf}\left(c_{key},c^{(i)}_a\right) $.
 Thus, we now end up with 
the following equation for the overall probability of a successful match considering all matching partners:
\begin{equation}
  f_{conf}(t,c_{key}, c^k) = \sum_{i=2}^k \left( (-1)^i \cdot (i-1) \cdot \sum_{c^{(i)} \in C^{(i)}_{k} }  \left( \prod_{j=1}^i f_{conf}\left(c_{key},c^{(i)}_j\right)  \right) \right) ,
  \label{eq:prob}
\end{equation}
where $C^{(i)}_{k}$ is the solution space for drawing subsets of $i$ cameras
from the available set of $k$ matching partners, $c^{(i)}$ is one of these subsets and 
$c^{(i)}_j$ is one camera of this subset and
$f_{conf}\left(c_{key},c^{(i)}_j\right)$ is the pair-wise MVS confidence for camera $c^{(i)}_j$
with the key camera $c_{key}$.
We compute this pair-wise MVS confidence by averaging the unary confidence values.
For each pair of images, it would be possible to extract these values with the random forest directly from the RGB images.
However for computational efficiency, we cache these values at the beginning of our prioritization approach (Section~\ref{sec:ic}).

In detail, we first discretized the unary MVS confidence function into 9 bins (1 bin per $5^\circ$ triangulation angle) and
precompute the confidence values on a regular grid with 8 pixel stride in the image as in~\citep{mostegel16b}.
% Further, we store  our view cluster ranking approach (Section~\ref{sec:ic}) additionally
% caches unary confidence predictions on a triangle basis.
Then we store the unary confidence values for each image that observes a triangle inside the triangle's data structure.
These unary confidence values are obtained by projecting the triangle into the precomputed confidence images 
and averaging all values within the triangle for each bin separately.
This caching scheme precomputes all necessary unary confidence values and 
turns the confidence prediction task in our prioritization approach into simple and fast look-up operations.
% Through this caching scheme, we avoid redundant computations in our prioritization approach (Section~\ref{sec:ic})
% In this way, the pair-wise MVS confidence (between two images) can be obtained by two simple look up operations within the triangle (one for each image)
% and then averaging the precomputed unary confidence predictions for each camera.
